Quantum Perfect Matchings

We investigate quantum and nonsignaling generalizations of perfect matchings in graphs using nonlocal games. Specifically, we introduce nonlocal games that test for $L$-perfect matchings in bipartite graphs, perfect matchings in general graphs and hypergraphs, and fractional perfect matchings. Our definitions come from the fact that these games are classical property tests for the corresponding matching conditions. We use the existence of perfect quantum and nonsignaling strategies for these games to define quantum and nonsignaling versions of perfect matchings. Finally, we provide characterizations of when graphs exhibit these extended properties: - For nonsignaling matchings, we give a complete combinatorial characterizations. In particular, a graph has a nonsignaling perfect matching if and only if it admits a fractional perfect matching that has bounded value on triangles. \item In bipartite graphs, the nonsignaling $L$-perfect matching property is achieved exactly when the left component of the graph can be split into two disjoint subgraphs: one with a classical $L$-perfect matching and another with left-degree 2. - In the quantum setting, we show that complete graphs $K_n$ with odd $n \geq 7$ have quantum perfect matchings. We prove that a graph has a quantum perfect matching if and only if the quantum independence number of its line graph is maximal, extending a classical relationship between perfect matchings and line graph independence numbers. - For bipartite graphs, we establish that the $L$-perfect matching game does not exhibit quantum pseudotelepathy, but we characterize the quantum advantage for complete bipartite graphs $K_{n,2}$. - Additionally, we prove that deciding quantum perfect matchings in hypergraphs is undecidable and leave open the question of its complexity in graphs.

==> sections/ConstrainedIso.tex <==
\section{Constrained Isomorphism Games} \label{conIso}
Here we provide a natural simultaneous generalization of both the bipartite matching and isomorphism games. 

\begin{defn}
Given two graphs $G = (V_G, E_G)$ and $H = (V_H, E_H)$ and the bipartite constraint graph $C = (V_G,V_H,E_C)$ we define the synchronous game $ISO_C(G,H)$. The game has question set $V_G$ and answer set $V_H$ with the uniform distribution. The players win if on questions $(x_1,x_2)$ they respond with $(y_1, y_2)$ such that
\begin{enumerate}
    \item (consistency) if $x_1 = x_2$ then $y_1 = y_2$
    \item (adjacency) if $x_1 \sim x_2$ then $y_1 \sim y_2$
    \item (non-adjacency) if $x_1 \nsim x_2$ then $y_1 \nsim y_2$
    \item (isomorphism constraint) $(x_1,y_1), (x_2,y_2) \in E_C$ 
\end{enumerate}
\end{defn}

Then bipartite matching games correspond to the above game where the graphs $G$ and $H$ consist of lone vertices and the constraint graph $C$ is the bipartite graph in the matching game. 

Similarly the Isomorphism games between graphs $G$ and $H$ correspond to the above game with the same graphs and the fully connected constraint bipartite graph.

In between these two extremes we get a set of interesting games where Alice and Bob attempt to convince a verifier that there exists an isomorphism between two graphs that obeys certain constraints encoded in the bipartite graph $C$. 

\todo{Todo. Play around with these games and try to find some interesting examples}
